Sensing Micro-colloid Concentration by Spectral Impedance Measurements and Relaxation Times Analysis

This paper presents an attractive method towards sensing and quantifying the concentration of dielectric particles suspended in a highly conductive medium. Fast electrical impedance spectroscopy (EIS) measurements were performed, based on an electrochemical setup and a non-parametric unbiased estimator. The impedance data are then mapped from the frequency domain to a time constant domain via the distribution of relaxation times (DRT) model. It is shown that application of DRT can systematically give a distribution function which is directly related with the concentration of micro-colloid samples. As a result, the samples were characterized by high sensitivity and resolution.

==> macrosetup.tex <==
%% Custom commands
%% ===============

%% Special characters for number sets, e.g. real or complex numbers.
\newcommand{\C}{\mathbb{C}}
\newcommand{\K}{\mathbb{K}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\X}{\mathbb{X}}
\newcommand{\I}{\mathbb{I}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\V}{\mathbb{V}}
%% Fixed/scaling delimiter examples (see mathtools documentation)
\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert}

%% Use the alternative epsilon per default and define the old one as \oldepsilon
\let\oldepsilon\epsilon
\renewcommand{\epsilon}{\ensuremath\varepsilon}

%% Also set the alternate phi as default.
\let\oldphi\phi
\renewcommand{\phi}{\ensuremath{\varphi}}

\renewcommand{\Re}{\textnormal{Re\,}}
\renewcommand{\Im}{\textnormal{Im\,}}
%% Hilbert Spaces
\newcommand{\Asp}{\mathcal{A}}
\newcommand{\Csp}{\mathcal{C}}
\newcommand{\Bsp}{\mathcal{B}}
\newcommand{\Dsp}{\mathcal{D}}
\newcommand{\Esp}{\mathcal{E}}
\newcommand{\Fsp}{\mathcal{F}}
\newcommand{\Gsp}{\mathcal{G}}
\newcommand{\Hsp}{\mathcal{H}}
\newcommand{\Isp}{\mathcal{I}}
\newcommand{\Ksp}{\mathcal{K}}
\newcommand{\Lsp}{\mathcal{L}}
\newcommand{\Pspa}{\mathcal{P}}
\newcommand{\Qsp}{\mathcal{Q}}
\newcommand{\Ssp}{\mathcal{S}}
\newcommand{\Tsp}{\mathcal{T}}
\newcommand{\Usp}{\mathcal{U}}
\newcommand{\Vsp}{\mathcal{V}}
\newcommand{\Wsp}{\mathcal{W}}
\newcommand{\Msp}{\mathcal{M}}
\newcommand{\Nsp}{\mathcal{N}}
\newcommand{\Psp}{\mathcal{P}}
\newcommand{\Rsp}{\mathcal{R}}
\newcommand{\Xsp}{\mathcal{X}}
\newcommand{\Ysp}{\mathcal{Y}}
\newcommand{\Zsp}{\mathcal{Z}}

\renewcommand{\abs}[1]{\left| #1\right|}

\newcommand{\hZdrt}{\hat{Z}_{\text{DRT}}}
\newcommand{\hZcc}{\hat{Z}_{\text{CC}}}
\newcommand{\Zdrt}{Z_{\text{DRT}}}
\newcommand{\Zcc}{Z_{\text{CC}}}
\newcommand{\Zre}{Z_{\Re}}
\newcommand{\Zim}{Z_{\Im}}
\newcommand{\w}{\omega}


\newcommand{\argminE}{\mathop{\mathrm{argmin}}} 
\newcommand{\RED}[1]{\textcolor{red}{#1}}
\newcommand{\ZBIO}{Z_{\textnormal{BIO}}}
\newcommand{\HZBIO}{\hat{Z}_{\textnormal{BIO}}}
\newcommand{\ZDRT}{Z_{\textnormal{DRT}}}
\newcommand{\eq}{\triangleq}
\newcommand{\re}{\Re}
\newcommand{\im}{\Im}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}


\newcommand{\bz}{\boldsymbol{z}}
\newcommand{\bZ}{\boldsymbol{Z}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
